CAPRI-FAIR: Integration of Multi-sided Fairness in Contextual POI Recommendation Framework

Point-of-interest (POI) recommendation considers spatio-temporal factors like distance, peak hours, and user check-ins. Given their influence on both consumer experience and POI business, it's crucial to consider fairness from multiple perspectives. Unfortunately, these systems often provide less accurate recommendations to inactive users and less exposure to unpopular POIs. This paper develops a post-filter method that includes provider and consumer fairness in existing models, aiming to balance fairness metrics like item exposure with performance metrics such as precision and distance. Experiments show that a linear scoring model for provider fairness in re-scoring items offers the best balance between performance and long-tail exposure, sometimes without much precision loss. Addressing consumer fairness by recommending more popular POIs to inactive users increased precision in some models and datasets. However, combinations that reached the Pareto front of consumer and provider fairness resulted in the lowest precision values, highlighting that tradeoffs depend greatly on the model and dataset.

==> sections/copy_old_meth.tex <==
\textbf{Datasets}\\
For training, we will use the Gowalla and Yelp datasets. Both these datasets are used in \cite{p50-werneck2021points, p66-rahmani2022role} as a benchmark because of their greater feature sets, which allows more models to be compared. A similar preprocessing step will also be employed to remove POI's visited by less than 10 users, as well as users who have visited POI's less than 10 times. For the training, validation, and testing set split, a 70-20-10 split of each user's logs will be made.

Users will be divided according to activity, where the top 20\% of users will be assigned to the active group, and the rest to the inactive group. Likewise, the process in \cite{p15-naghiaei2022cpfair} can be followed to designate item groups, where items are split into short-head and long-tail groups based on their popularity, with the top 20\% of items by popularity being designated in the short-head group. Statistics on the 2 datasets, including these divisions, are shown below in Table \ref{table:dataset-stats}.

\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c c c c|c c c|}
    \hline
    Dataset & Users & POIs & Checkins & Sparsity & Active/Inactive Users & Long-tail/Short-head POIs & Long-tail/Short-head Checkins \\
    \hline
    Yelp & 7135 & 16621 & 774320 & 0.65\% & 1427 / 5708 & 12413 / 3162 & 280255 / 494065 \\
    Gowalla & 5628 & 31803 & 483846 & 0.27\% & 1125 / 4503 & 24700 / 6243 & 164459 / 319387 \\
    \hline
\end{tabular}
}
\caption{Dataset statistical}
\label{table:dataset-stats}
\end{table*}

\textbf{Evaluation Metrics}\\
For evaluation, we will primarily use Precision@k as our accuracy metric, as this is the most commonly used one in the field. Precision@k simply checks if the target POI to be predicted lies in the first $k$ entries in the recommendation list, which for a use case where hits (i.e. visits to a POI) are sparse, would suffice.

For evaluating user and item fairness, we can measure both Precision and Exposure across the user and item groups respectively. For a single measurable metric of fairness, the Generalized Cross-Entropy (GCE) of the metric distribution can be used for both cases \cite{p31-rahmani2022unfairness} \cite{p55-deldjoo2021flexible}. For categorical attributes $a \in A$ with respect to which fairness will be computed, the GCE for a given model $m$ is defined as such:

\begin{equation}
    GCE(m, a) = \frac{1}{\beta \cdot (1 - \beta)}\Bigg[\sum_{a_j} p^\beta_f(a_j) p^{(1-\beta)}_m(a_j) - 1\Bigg]
\end{equation}

Here, $p_m$ and $p_f$ represent the metric distributions of the model outputs and a theoretical fair model, respectively. The index $\beta$ represents the index of the unfairness measure being used, which includes the Hellinger distance ($\beta = \frac{1}{2}$), Pearson's $\chi^2$ ($\beta = 2$), Kullback-Leibler divergence ($\lim_{\beta \rightarrow 1}$), and a few others. As mentioned in \cite{p55-deldjoo2021flexible}, the Pearson's $\chi^2$ measure is more robust to outliers, so a value of $\beta = 2$ will be used.

To adapt this GCE formulation to consumer fairness, we define a recommendation gain for each user based on the lists recommended to the user. Each of the POIs have an associated gain to them. In the case of recommendation hits or relevance, we can add 1 for each POI in each recommendation result that correspond to one visited by the user. We can define this similarly to the attention function used in calculating item exposure $a(p, P_R)$. If we define $\phi(u, p)$ as an indicator function which equals either 0 or 1 depending on whether or not the user has visited the POI, we can define the recommendation gain, as well as the overall metric distribution as follows:

\begin{equation}
    p_m(a_i) = \frac{1}{Z} \sum_{u \in U_{a_i}} rg_u = \frac{1}{Z} \sum_{u \in U_{a_i}} \sum_{P_{Ru} \subset P} \sum_{p \in P_{Ru}} \phi(u, p) \cdot a(p, P_{Ru})
\end{equation}

Note that $Z$ is a simple normalization factor which ensures that the sum of the metric distribution values equals 1. We can define a similar metric for provider fairness. We tweak the indicator function to indicate if a POI is in a recommendation list, and restate it as $\delta(p, P_{Ru})$. The resulting recommendation gain for POIs is as follows:

\begin{equation}
    p_m(a_i) = \frac{1}{Z} \sum_{i \in I_{a_i}} rg_i = \frac{1}{Z} \sum_{i \in I_{a_i}} \sum_{P_{Ru} \subset P} \delta(p, P_{Ru})
\end{equation}

Because of the constraints of the POI recommendation task, metrics with respect to these constraints can also be defined. For geographical distance, a simple average distance of recommended POIs to users may be employed.
\\
\\
\textbf{Benchmarking and Experimentation}\\
As a baseline, the proposed model will be compared with the 3 baseline methods defined in \cite{p70-tourani2023capri}: USG, GeoSoCa, and LORE, as these are the most commonly used baselines in the survey. The same datasets and benchmarking framework will be used and extended\footnote{https://anonymous.4open.science/r/CAPRI-7FA3/}.

To answer the set of research questions, we test the following hypotheses regarding the model's impact on the metrics:

\begin{enumerate}
    \item The choice of the exposure model used for provider fairness has a significant impact on its effect on model performance.
    \item The provider fairness factor can introduce a significant improvement to the long-tail item exposure, without similar or worse decreases to the model accuracy.
    \item The consumer fairness factor can introduce a significant improvement to precision for inactive users.
    \item Using a combination of provider and consumer fairness, significant improvements to the GCE fairness metrics can be achieved from the baseline.
\end{enumerate}

To answer the first research question regarding the impact of the exposure model choice on the provider fairness factor's impact, the 3 models (power law, linear, and logistic) will be assessed on the benchmark, across values of $\alpha = 0, 0.25, 0.5, 1.0$, taking note of precision and long-tail exposure for $k = 10$ as the main metrics. A test for significance will be employed in order to see if the model choice has a significant impact on the metrics. From here, the best option will be adopted for the next experiments.

For the second and third hypothesis, the provider fairness and consumer fairness factors will be assessed separately over a range of weights from 0 to 1, on the aforementioned metrics for performance, fairness, and distance. At a weight of 1, the weight of the factor is the same as that of the original score, thus the fairness factor comprises $\frac{1}{2}$ of the score. Plots for $k = 10$ will be included in the results.

For the last hypothesis, a total weight of 1 will be shared between the 2 factors, and they will be distributed between the 2 of them in varying weights. The same metrics will be plotted to see the impact of varying such parameters, for values of $k = 5, 10, 20$.

% \subsubsection{TO DELETE}

% \begin{enumerate}
%     \item ProviderModel x ProviderAlpha (0-0.25-0.5-0.75-1), precision + NDCG + exposure
%     \item ProviderAlpha (0...1) x k (5-10-20), all metrics
%     \item ConsumerBeta (0...1) x k (5-10-20), all metrics
%     \item PA+CB (0/0.5 , 0.1/0.4 , 0.2/0.3 , 0.3/0.2 , 0.4/0.1 , 0.5/0) x k (5-10-20)
% \end{enumerate}

==> sections/copy_old_result.tex <==
\subsection{Comparison between exposure models}

The benchmark models were run first without modification, then while slowly increasing the provider fairness factor's coefficient $\alpha$ from 0.1 to 1.0. The impact of the provider fairness model used is first assessed by taking note of its impact on the precision and exposure metrics for the long tail, which it is aiming to improve. The results are shown below in Table \ref{table:prec-ltexp-exposuremodel-yelp}.

\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c c||c c c c c|c c c c c|}
    \hline
    Dataset & Model & Exposure Model & \multicolumn{5}{c|}{Precision} & \multicolumn{5}{c|}{Long-tail Exposure} \\
    & & & 0 & 0.25 & 0.50 & 0.75 & 1 & 0 & 0.25 & 0.50 & 0.75 & 1 \\
    \hline\hline
    Yelp & GeoSoCa & Linear & 0.0225 & 0.0134 & \textbf{0.0117} & \textbf{0.0111} & \textbf{0.0107} & 1.7010 & \textbf{3.4467} & 4.1525 & 4.5026 & 4.6888 \\
    & & Logistic & 0.0225 & \textbf{0.0173} & 0.0089 & 0.0073 & 0.0073 & 1.7010 & 3.0696 & \textbf{4.5693} & \textbf{4.6969} & \textbf{4.6970} \\
    & & PowerLaw & 0.0225 & 0.0137 & 0.0109 & 0.0096 & 0.0081 & 1.7010 & 3.1636 & 3.5278 & 2.5025 & 1.8429 \\
    \hline
    & LORE & Linear & 0.0230 & 0.0179 & \textbf{0.0147} & \textbf{0.0132} & \textbf{0.0124} & 1.5290 & 2.7975 & 3.6141 & 4.1361 & 4.4426 \\
    & & Logistic & 0.0230 & 0.0183 & 0.0096 & 0.0074 & 0.0072 & 1.5290 & \textbf{3.4217} & \textbf{4.8180} & \textbf{4.9503} & \textbf{4.9565} \\
    & & PowerLaw & 0.0230 & \textbf{0.0196} & 0.0136 & 0.0106 & 0.0082 & 1.5290 & 2.2284 & 2.1647 & 1.8887 & 1.5768 \\
    \hline
    & USG & Linear & 0.0297 & \textbf{0.0314} & 0.0278 & \textbf{0.0228} & \textbf{0.0186} & 0.0077 & 0.0341 & 0.5424 & 1.8214 & 3.0765 \\
    & & Logistic & 0.0297 & 0.0296 & 0.0257 & 0.0123 & 0.0042 & 0.0077 & \textbf{0.0461} & \textbf{1.1532} & \textbf{4.5227} & \textbf{5.6810} \\
    & & PowerLaw & 0.0297 & 0.0300 & \textbf{0.0291} & 0.0152 & 0.0036 & 0.0077 & 0.0209 & 0.2791 & 2.9418 & 3.9288 \\
    \hline\hline
    Gowalla & GeoSoCa & Linear & 0.0381 & 0.0300 & \textbf{0.0287} & \textbf{0.0274} & \textbf{0.0266} & 0.7990 & 0.9796 & 1.0734 & 1.1626 & 1.2465 \\
     & & Logistic & 0.0381 & \textbf{0.0316} & 0.0182 & 0.0140 & 0.0132 & 0.7990 & 1.2142 & \textbf{1.9263} & \textbf{2.0336} & 2.0459 \\
     & & PowerLaw & 0.0381 & 0.0277 & 0.0242 & 0.0222 & 0.0203 & 0.7990 & \textbf{1.3231} & 1.8073 & 2.0207 & \textbf{2.0636} \\
    \hline
    & LORE & Linear & 0.0482 & \textbf{0.0427} & \textbf{0.0405} & \textbf{0.0389} & \textbf{0.0378} & 0.7354 & 0.9356 & 1.0757 & 1.1958 & 1.2961 \\
     & & Logistic & 0.0482 & 0.0283 & 0.0149 & 0.0127 & 0.0125 & 0.7354 & \textbf{1.6326} & \textbf{2.0425} & \textbf{2.0815} & \textbf{2.0842} \\
     & & PowerLaw & 0.0482 & 0.0392 & 0.0260 & 0.0191 & 0.0156 & 0.7354 & 1.2983 & 1.6527 & 1.7724 & 1.7771 \\
    \hline
    & USG & Linear & 0.0514 & 0.0504 & \textbf{0.0477} & \textbf{0.0446} & \textbf{0.0424} & 0.0766 & 0.1056 & 0.1567 & 0.2523 & 0.3689 \\
     & & Logistic & 0.0514 & 0.0500 & 0.0334 & 0.0195 & 0.0103 & 0.0766 & \textbf{0.2319} & \textbf{1.4315} & \textbf{2.0190} & \textbf{2.2654} \\
     & & PowerLaw & 0.0514 & \textbf{0.0525} & 0.0468 & 0.0293 & 0.0158 & 0.0766 & 0.1513 & 0.7876 & 1.6531 & 2.0789 \\
    \hline
\end{tabular}
}
\caption{Precision and Long-tail Exposure for different Provider Fairness factor weights and Exposure models used.}
\label{table:prec-ltexp-exposuremodel-yelp}
\end{table*}

The score of the best-performing exposure model for the metric is highlighted in bold. For precision, which is the accuracy or performance metric of choice here, the linear exposure model performs the best in most cases. This makes sense as it doesn't punish even slightly popular POIs as harshly as the other models, as shown by the curves in the Figure \ref{fig:different-models} above. Likewise, the logistic model performs the best in terms of exposure to the long-tail, which makes sense as it only provides weights to only the least popular POIs. Note however, that the linear model still provides a reasonable increase to the long-tail exposure as the weight is increased. The power law model, however, seems to perform the worst for the GeoSoCa and LORE models, and even decreases past a certain weight. Running a Kruskal-Wallis test on the precision and exposure values reveals a statistically significant difference in metric values among the 3 exposure models, starting from a factor weight of $\alpha = 0.5$, indicating that the choice of the exposure model does make a difference in the precision and long-tail exposure metrics. Moving forward, we can now use the linear model for the provider fairness factor, as it offers the highest precision values and permits a moderate long-tail exposure.

\subsection{Impact of the provider fairness factor}

Now that the linear model was selected as the provider fairness factor model for further experiments, its impact on the performance, fairness, and geographical metrics can be assessed with further scrutiny. The impact on our main accuracy metric Precision@10 is shown in Figure \ref{fig:prec-provfactor}. Intuitively, prioritizing the interests of the providers by increasing the provider fairness factor correlates with a decrease in accuracy metrics, however USG seems to react positively for smaller values of the factor weight, where the accuracy metrics even go up. On the other hand, GeoSoCa and LORE seem to experience sharp decreases for the same smaller values. This unfortunately means that when using these 2 models, even a small increase in the provider factor can lead to significant decreases to precision, especially for the GeoSoCa model, where an increase of $\alpha$ from 0 to 0.1 means a decrease in precision from 2.3\% to 1.7\%, which is a large 25\% decrease.

% \begin{figure}[!htb]
%     \centering
%     \makebox[\textwidth][c]{
%         \begin{minipage}{0.35\paperwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/results_2/precision_vs_provider_alpha.png}
%             \caption{Precision@10}
%             \label{fig:prec-provfactor}
%         \end{minipage}
%         \begin{minipage}{0.35\paperwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/results_2/ndcg_vs_provider_alpha.png}
%             \caption{NDCG@10}
%             \label{fig:ndcg-provfactor}
%         \end{minipage}
%     }
%     \caption{Accuracy metrics v.s. Provider fairness factor $\alpha$}
%     \label{fig:acc-provfactor}
% \end{figure}

The geographical aspect of POI recommendation means that the impact on the median distance of POIs to the average position of the user should also be considered. As shown in Figure \ref{fig:mmd-provider-fairness}, the distance doesn't vary significantly as the factor's weight is increase, and it even decreases for the Gowalla dataset. When we consider that a majority of POIs would be distant from any specific point in the map, it would be an initial guess to assume that if we give too much weight to the long tail, we give more weight to further and further POIs, which could increase this metric, however it might also be the case where unpopular POIs could be distributed even close to where the user visits.

\begin{figure*}[!htb]
    \centering
    \makebox[\textwidth][c]{
        \begin{minipage}{0.35\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/results_2/precision_vs_provider_alpha.png}
            \caption{Precision@10 v.s. Provider fairness factor $\alpha$}
            \label{fig:prec-provfactor}
        \end{minipage}
        \begin{minipage}{0.35\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/results_2/mean_median_distance_vs_provider_alpha.png}
            \caption{Median POI distance v.s. Provider fairness factor $\alpha$}
            \label{fig:mmd-provider-fairness}
        \end{minipage}
    }
\end{figure*}


Most importantly, we see that it does help with exposure to the long-tail POIs, who under the normal regime experience very low exposure rates of 1-2 recommendation appearances overall, as compared with 15-20 recommendation appearances for the short-head POIs. For USG, this exposure is as low as near-0 by default. As shown in Figures \ref{fig:exp-longtail-provfactor} and \ref{fig:exp-shorthead-provfactor}, an increase in the factor's weight increases the long-tail exposure, and accordingly decreases the short-head exposure, where at $\alpha = 0.5$, the increase in long-tail exposure reaches a 1.4-times increase from the default for GeoSoCa and LORE, and an even larger one from 0 to 0.54 for the USG model. A similar pattern to the precision metric can be seen, where for USG the metric isn't affected until a certain point where the precision and short-head exposure decreases, and the long-tail exposure similarly increases. Similarly, the long-tail exposure for the GeoSoCa and LORE models also exhibit sharp changes. This displays the correlation between the increase in long-tail exposure and the decrease in overall precision.

\begin{figure*}[!htb]
    \centering
    \makebox[\textwidth][c]{
        \begin{minipage}{0.35\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/results_2/exposure_short_head_vs_provider_alpha.png}
            \caption{Exposure metrics for the Short head (top 20\%)}
            \label{fig:exp-shorthead-provfactor}
        \end{minipage}
        \begin{minipage}{0.35\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/results_2/exposure_long_tail_vs_provider_alpha.png}
            \caption{Exposure metrics for the Long tail (bottom 80\%)}
            \label{fig:exp-longtail-provfactor}
        \end{minipage}
    }
\end{figure*}

When we run a Wilcoxon signed rank test to test the precision and long-tail exposure metrics for each user and POI, before and after adding the provider fairness factor, we see that even the addition of the factor with a weight of $\alpha = 0.1$ causes a significant change in almost all cases, barring only the change in USG's precision over the Gowalla dataset. For GeoSoCa and LORE, this change is a decrease in precision, however for USG it is the slight increase in precision at the start. This shows that the fairness factor does have a significant impact on the metrics of interest.

% Another way of visualizing this fairness impact is shown below in Figure \ref{fig:prov-fairness-scatter}, which plots the different results in a plot of long-tail exposure v.s. short-head exposure, and where the darker points represent higher values of $\alpha$. Here, the blue line represents the $y=x$ line where equality is achieved, in that the exposure is equal between the 2 groups. As expected, the increase in weight does in fact get it closer to equality. Here, it can be also seen that the factor has a much higher impact on the Yelp dataset, where the baselines are a lot more imbalanced but the points quickly reach the blue line.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.70\textwidth]{images/provider_fairness_plot.png}
%     \caption{Plot of exposure between the 2 provider groups. The blue line represents perfect fairness where the values are the same.}
%     \label{fig:prov-fairness-scatter}
% \end{figure}


\subsection{Impact of the consumer fairness factor}

Increasing the weight of the consumer fairness factor will hopefully increase the accuracy metrics of the model, as while active users would be unaffected, inactive users will hopefully be recommended POIs that they are more likely to visit. Figures \ref{fig:prec-consfactor} and \ref{fig:prec-consfactor-inactive} shows that when this factor's weight is increased, the precision of the GeoSoCa and LORE models increase from 2.3\% to 2.6\% in the Yelp dataset, and similarly increases at first for the first half of values for $\beta$. However, in most other cases, the performance actually degrades, especially with the USG model which goes from 3.0\% to 2.8\%. This could be because the most popular recommendations aren't necessarily the ones most personalized to the user. When we run a Wilcoxon signed rank test as with the previous section, we also see that even the addition of the factor with a weight of $\beta = 0.1$ causes a significant change in almost all cases (once again only barring the change in USG's precision over both datasets), showing that this factor does have a significant impact.

Interestingly enough, this method causes an increase in the median distance of recommendations, as shown in Figure \ref{fig:mmd-cons-fairness}, which is counter to the strategy of recommending POIs nearby ones that were already visited. This could be due to the difference in evaluation, where the metric considers distance from the user's average location.

% \begin{figure}[!htb]
%     \centering
%     \makebox[\textwidth][c]{
%         \begin{minipage}{0.35\paperwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/results_3/precision_vs_consumer_beta.png}
%             \caption{Precision@10}
%             \label{fig:prec-consfactor}
%         \end{minipage}
%         \begin{minipage}{0.35\paperwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/results_3/ndcg_vs_consumer_beta.png}
%             \caption{NDCG@10}
%             \label{fig:ndcg-consfactor}
%         \end{minipage}
%     }
%     \makebox[\textwidth][c]{
%         \begin{minipage}{0.35\paperwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/results_3/precision_inactive_users_vs_consumer_beta.png}
%             \caption{Precision@10 for inactive users}
%             \label{fig:prec-consfactor-inactive}
%         \end{minipage}
%     }
%     \caption{Accuracy metrics v.s. Consumer fairness factor $\beta$}
%     \label{fig:acc-consfactor}
% \end{figure}

\begin{figure}[!htb]
    \centering
    \makebox[\textwidth][c]{
        \begin{minipage}{0.35\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/results_3/precision_vs_consumer_beta.png}
            \caption{Precision@10 v.s. Consumer fairness factor $\beta$}
            \label{fig:prec-consfactor}
        \end{minipage}
        \begin{minipage}{0.35\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/results_3/precision_inactive_users_vs_consumer_beta.png}
            \caption{Precision@10 for inactive users}
            \label{fig:prec-consfactor-inactive}
        \end{minipage}
    }
\end{figure}


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.5\textwidth]{images/results_3/mean_median_distance_vs_consumer_beta.png}
    \caption{Median POI distance v.s. Consumer fairness factor $\beta$}
    \label{fig:mmd-cons-fairness}
\end{figure}

% If we use the same scatter visualization for consumer fairness in Figure \ref{fig:cons-fairness-scatter}, we see that the impact is a lot less directly positive, and the unfairness is much larger, as the points are further away from the blue line. For some models like USG, the factor even increases unfairness, as we also see in the plots above. Note that, because the strategy only affects inactive users, the factor does not affect the precision for active users, hence the points staying in the same line parallel to the x-axis.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.70\textwidth]{images/consumer_fairness_plot.png}
%     \caption{Plot of precision between the 2 consumer groups. The blue line represents perfect fairness where the values are the same.}
%     \label{fig:cons-fairness-scatter}
% \end{figure}


\subsection{Tradeoff between provider and consumer fairness}

Now that we have the 2 fairness factors to consider, the next question is to see how a combination of the 2 will affect the same metrics. For the graphs, a weight of 1.0 is shared between the consumer and provider factors. Although we see that even a high consumer fairness factor will decrease accuracy metrics for the USG model, it still affects it less than a high provider fairness factor. For GeoSoCa and LORE in particular, the performance increases as more weight is given to consumer fairness, and away from producer fairness. USG shows a peak midway, at a weight distribution of $\alpha = 0.3, \beta = 0.7$ for the Yelp dataset, and $\alpha = 0.2, \beta = 0.8$ for the Gowalla dataset.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.5\textwidth]{images/results_4/precision_vs_tradeoff.png}
    \caption{Precision@10 v.s. Tradeoff between consumer and provider fairness factors}
    \label{fig:prec-bothfactor}
\end{figure}

When looking at the fairness metrics for both long-tail items and inactive users, we see the expected changes, where an increase in the consumer fairness factor's weight corresponds to a decrease in long-tail exposure, and an increase in precision for inactive users. In particular, even a small addition of consumer fairness weight can cause a large decrease in exposure, especially for USG, where a weight of $\beta = 0.2$ can cause a 3-fold decrease in long-tail exposure.

\begin{figure*}[!htb]
    \centering
    \makebox[\textwidth][c]{
        \begin{minipage}{0.35\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/results_4/exposure_long_tail_vs_tradeoff.png}
            \caption{Exposure for Long tail items (bottom 80\%)}
            \label{fig:explt-bothfactor}
        \end{minipage}
        \begin{minipage}{0.35\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/results_4/precision_inactive_users_vs_tradeoff.png}
            \caption{Precision@10 for inactive users (bottom 80\%)}
            \label{fig:precinactive-bothfactor}
        \end{minipage}
    }
\end{figure*}

A closer look at the GCE metrics for fairness for different tradeoffs is tabulated below, including results when a smaller total weight is given to fairness, which might be a more realistic formulation in order to avoid large decreases in performance.

\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{|c c||c c c|c c c|c c c|c c c|}
        \hline
        Model & Fairness Weights & \multicolumn{3}{c|}{Precision} & \multicolumn{3}{c|}{Item fairness GCE} & \multicolumn{3}{c|}{User fairness GCE} & \multicolumn{3}{c|}{Mean median distance} \\
        & $(\alpha, \beta)$ & @5 & @10 & @20 & @5 & @10 & @20 & @5 & @10 & @20 & @5 & @10 & @20 \\
        \hline\hline
        GeoSoCa & (0.0, 0.0) & 0.02537 & 0.02252 & 0.01901 & -0.67755 & -0.59265 & -0.5093 & -0.14592 & -0.14098 & -0.14513 & 101.17249 & 100.45895 & 99.29816 \\
         & (0.0, 0.5) & 0.0291 & 0.02537 & 0.02159 & -5.89764 & -4.54826 & -3.34275 & -0.09071 & -0.09333 & -0.09345 & 100.33198 & 99.73246 & 99.80617 \\
         & (0.0, 1.0) & \textbf{0.02949} & \textbf{0.02562} & \textbf{0.02195} & -9.9195 & -8.07117 & -6.32284 & -0.08641 & -0.09007 & -0.08808 & 102.35795 & 102.48056 & 101.51285 \\
         & (0.25, 0.25) & 0.0169 & 0.01598 & 0.01399 & -0.6379 & -0.56611 & -0.49125 & -0.04459 & -0.03675 & -0.04917 & 98.60541 & 97.4856 & 97.20788 \\
         & (0.5, 0.0) & 0.01345 & 0.01173 & 0.0108 & \textbf{-0.00053} & \textbf{-0.00334} & \textbf{-0.00759} & -0.06675 & -0.06383 & -0.06583 & \textbf{96.86406} & \textbf{96.87758} & \textbf{97.11985} \\
         & (0.5, 0.5) & 0.01603 & 0.01453 & 0.01282 & -0.57984 & -0.52849 & -0.46714 & \textbf{-0.03134} & \textbf{-0.02418} & \textbf{-0.03132} & 99.0131 & 98.98704 & 98.47554 \\
         & (1.0, 0.0) & 0.01233 & 0.01071 & 0.00955 & -0.06374 & -0.03787 & -0.02046 & -0.03798 & -0.06055 & -0.06478 & 97.4033 & 97.37404 & 97.60246 \\
         \hline
        LORE & (0.0, 0.0) & 0.0252 & 0.023 & 0.02049 & -0.765 & -0.72147 & -0.63036 & -0.12356 & -0.13072 & -0.13131 & 97.35154 & 96.37364 & 96.67669 \\
         & (0.0, 0.5) & 0.02826 & 0.02572 & 0.02305 & -3.19637 & -3.20054 & -3.06965 & -0.08243 & -0.08841 & -0.08695 & 98.88016 & 98.2366 & 98.32551 \\
         & (0.0, 1.0) & \textbf{0.02929} & \textbf{0.02657} & \textbf{0.02341} & -6.95594 & -6.77278 & -6.08884 & -0.07205 & -0.07841 & -0.0821 & 100.45197 & 99.56773 & 99.89955 \\
         & (0.25, 0.25) & 0.02105 & 0.01964 & 0.01687 & -0.58276 & -0.57503 & -0.53311 & -0.09777 & -0.09092 & -0.0879 & 97.48547 & 96.56786 & 96.24566 \\
         & (0.5, 0.0) & 0.01606 & 0.0147 & 0.01261 & -0.07092 & -0.05139 & -0.0277 & -0.1151 & -0.10619 & -0.11235 & \textbf{96.45963} & \textbf{95.95741} & \textbf{95.6067} \\
         & (0.5, 0.5) & 0.01844 & 0.01755 & 0.01499 & -0.5067 & -0.50162 & -0.47727 & \textbf{-0.06978} & \textbf{-0.0547} & \textbf{-0.05941} & 97.19982 & 96.48961 & 95.97415 \\
         & (1.0, 0.0) & 0.01407 & 0.0124 & 0.01064 & \textbf{-0.0} & \textbf{-0.00197} & \textbf{-0.01268} & -0.0963 & -0.0968 & -0.10213 & 96.85222 & 96.23217 & 95.69327 \\
         \hline
        USG & (0.0, 0.0) & 0.03397 & 0.02968 & 0.02491 & -404.16486 & -235.5631 & -100.90804 & -0.05906 & -0.07079 & -0.08213 & 115.49726 & 115.60542 & 114.38432 \\
         & (0.0, 0.5) & 0.03324 & 0.02882 & 0.02424 & -595.83844 & -552.20543 & -267.68722 & -0.06434 & -0.07915 & -0.09065 & 117.46961 & 115.80121 & 116.1397 \\
         & (0.0, 1.0) & 0.03263 & 0.02804 & 0.02374 & -707.64802 & -665.99347 & -419.15168 & -0.06917 & -0.08743 & -0.09763 & 120.61967 & 119.56118 & 118.70201 \\
         & (0.25, 0.25) & \textbf{0.03518} & \textbf{0.031} & \textbf{0.02639} & -182.2632 & -124.02658 & -67.06192 & -0.05818 & -0.08549 & -0.09072 & 112.82197 & 113.71123 & 113.15953 \\
         & (0.5, 0.0) & 0.03083 & 0.02783 & 0.02346 & -3.26253 & -2.88418 & -2.31393 & -0.05556 & -0.06852 & -0.07835 & 112.54663 & 113.1397 & 113.10282 \\
         & (0.5, 0.5) & 0.0317 & 0.0284 & 0.02397 & -13.47004 & -11.9686 & -9.91389 & -0.04953 & -0.06343 & -0.07234 & \textbf{112.05213} & 113.48431 & 113.014 \\
         & (1.0, 0.0) & 0.02094 & 0.01857 & 0.01501 & \textbf{-0.16983} & \textbf{-0.13466} & \textbf{-0.09566} & \textbf{-0.02918} & \textbf{-0.04137} & \textbf{-0.05436} & 112.63371 & \textbf{112.67297} & \textbf{110.77933} \\
        \hline
    \end{tabular}
}
\caption{Precision, GCE, and Mean median distance metrics with respect to different weights for providers and consumers. Yelp dataset.}
\label{table:metrics-with-tradeoffs-yelp}
\end{table*}

In particular, both GeoSoCa and LORE achieve the highest precision when all the weight is given to the consumer fairness factor, which unsurprisingly works against provider fairness in this example. USG, however, achieves the highest performance when only little weight is equally given to the 2 factors. The method's generally different reception to the fairness factors, and higher baseline performance, could be due to its incorporation of interaction data in its user-based collaborative filtering module, as this is one method that isn't shared with GeoSoCa or LORE.

With regards to item fairness, USG experiences the most issue with item fairness in this case, where it provides barely any exposure to the long-tail. Unsurprisingly, increasing only the provider fairness weight provides the best results. For user fairness, however, the best results were achieved with a mixture of both factors, suggesting that this strategy for attempting to improve the recommendations for inactive users may be ineffective. Finally, mean median distance seems less affected, with changes constituting a smaller percent. Nevertheless, it seems like provider fairness actually improves this metric, with all models having the best results when all the provided weight is given to the provider metric.

We can summarize these tables into a scatterplot that plots the tradeoff between the user precision GCE and the item exposure GCE metrics, while using color to denote precision, and shape to differentiate between models and values of $k$. These 2 plots are shown below in Figure \ref{fig:tradeoff-scatter} for both the Yelp and Gowalla datasets. In the left plot, we can see that the pareto front with respect to GCE users and GCE items, with goes around the upper right region of the plot, does not optimize for precision, and in fact consists of points that acheive low precision. Another thing to note is that the USG model seems to achieve the best precision, but at the cost of GCE for items. Luckily, this model as we've seen before is receptive to the provider fairness factor, even if its fairness often pales in comparison to other models. In the right plot, we see a similar story where the pareto front consists of models that achieve low precision. However, the points are a lot more spread out in this dataset, and some models like LORE are able to achieve moderate precision with a nice balance of the 2 fairness measures. This shows that the dataset and chosen model plays a significant role in how these 2 factors affect the recommendation quality. Certain models can have different baseline fairness measures and can respond differently to weight increase, while certain datasets can have users and properties that require a different provider or consumer fairness strategy, causing differences in how the weights affect where in the fairness plot the point goes.

\begin{figure*}[!htb]
    \centering
    \makebox[\textwidth][c]{
        \begin{minipage}{0.25\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/tradeoff_scatter_yelp.png}
        \end{minipage}
        \begin{minipage}{0.25\paperwidth}
            \centering
            \includegraphics[width=\textwidth]{images/tradeoff_scatter_gowalla.png}
        \end{minipage}
    }
    \caption{Scatterplot showing the tradeoff between GCE for users, GCE for items, and precision}
    \label{fig:tradeoff-scatter}
\end{figure*}

==> sections/related_work.tex <==
\subsection{Fairness}

The topic of fairness has been a hot field of research as machine learning systems have become more and more influential to our lives, however even the mere definition of fairness has been under scrutiny for a long time. The original definition can be attributed to Aristotle's statement that "those who are equal should be treated equally", however this has since been extended to various definitions, to the point where the consolidation of multiple definitions has become a challenge in the fairness literature \cite{p6-mehrabi2021survey}. The simplest way to specify fairness definitions is to distinguish between individual and group fairness. Individual fairness requires that similar individuals must be treated similarly, a concept that derives directly from Aristotle's definition \cite{p46-dwork2012awareness}. Group fairness, on the other hand, requires that members of different groups must be treated similarly. The groups in question are often defined by some sensitive attribute $a_i$, which separates the user base into a protected or minority group and dominant or majority group. Some examples of sensitive attributes may include race or gender. \cite{p5-ekstrand2022fairness}

These considerations regarding fairness become more complicated when applied to recommender systems. For one, the ranking of items means that the decision to include one item is not independent of the decision to include another; they still need to be reconciled in a ranking where the first item may receive more exposure. Moreover, the results are personalized to and subjective for each user, making estimation of the model's utility for the user more complicated \cite{p5-ekstrand2022fairness}. Finally, there are simply more sides to consider. In \cite{p1-burke2018balanced}, Burke et. al. explored the concept of multi-stakeholder recommender systems, where the users to whom the recommendations are served are not the only class of stakeholders. Here, three broad classes were proposed: consumers (the users who receive the recommendations, and benefit from having their interests accounted for), providers (the ones who provide the recommended items, and benefit from having their items recommended), and the system (the ones behind the platform itself, and who benefits from other decisions such as recommending certain promoted items).

Consumer fairness is the definition of fairness that's easiest to conceptualize in recommender systems. In \cite{p45-li2021user}, Li et. al. groups users into advantaged and disadvantaged groups, and show that current approaches to recommender systems perform much better for advantaged users. The study aimed to alleviate this using a re-ranking approach, where the recommendation items are shuffled and re-ranked to improve fairness metrics. Provider fairness, on the other hand, is different in that providers are more passive in the recommendation task, so the consumer's recommendations must be tweaked to affect it \cite{p1-burke2018balanced}. This is common in scenarios where some form of market diversity or fair distribution of resources is desired among those that provide the items. This also helps maintain a healthy catalog and avoids monopolies. The most common way to measure provider fairness is with provider exposure, which is proportional to the number of times the provider's items appear in consumer recommendations \cite{p7-abdollahpouri2020multistakeholder}.

As mentioned earlier, the interests of consumers and providers can clash or otherwise be in opposition to each other. Patro et. al. \cite{p47-patro2020fairrec} suggests a notion of fairness that takes these 2 competing viewpoints in consideration, and aligns the problem to that of the fair allocation of goods in social choice theory. Naghiaei et. al. \cite{p15-naghiaei2022cpfair} also considered both consumer and provider fairness, however they instead modelled it as a joint objective towards which a mathematical optimization formulation was made. Re-ranking was then applied to the results of a recommendation to optimize for this objective.

\subsection{Point-of-Interest Recommendation}
When recommending points of interest to a user, one of the biggest considerations for the user is the location of the point relative to the user. Generally speaking, the closer the recommendations are to the user geographically, the better. Levandoski et. al. \cite{p48-levandoski2012lars} explored this concept by considering the spatial location of users and items in a collaborative filtering model for recommendation. Ye et. al. \cite{p10-ye2011exploiting} also considers factors such as user preference alongside geographical location. One property of POI recommendation is the sparsity of data, as users are likely to only ever visit few POIs. On that end, Zhang and Chow \cite{p53-zhang2015geosoca} also explored the usage of geographical correlations, along with social and categorical correlations as well. Lian et. al. \cite{p54-lian2014geomf} addresses this by incorporating the spatial clustering of activity into a matrix factorization model.

The topic of fairness has also been addressed in the context of POI recommendation. In terms of provider fairness, Banerjee et. al. \cite{p39-banerjee2020analyzing} looks into how these systems can propagate exposure bias, where some providers and POIs receive significantly less exposure. Patro et. al. \cite{p2-patro2020towards} resolves this by modelling POI exposure as an objective in an optimization problem. The field of tourism recommender systems also often considers fairness and sustainability, with some studies considering the environment as a stakeholder, and its sustainability as an objective \cite{p37-banerjee2023fairness} \cite{p38-merinov2022sustainability}. Finally, while only fairness-adjacent, there have been studies that considered other beyond-accuracy metrics as well. Han and Yamana \cite{p57-han2017geographical} defined a concept of proportional geographical diversification which aimed to geographically spread out recommended POIs. Zhang et. al. \cite{p60-zhang2021snpr} focused on recommmendation serendipity, which can be thought of as correlated with item exposure fairness, while Rahmani et. al. \cite{p66-rahmani2022role} proposed a context fusion method that aimed to address beyond-accuracy and fairness.

As mentioned before, the balance of both consumer and provider fairness remains an important consideration for point-of-interest recommendation systems. Patro et. al. \cite{p2-patro2020towards} explored the multi-objective paradigm, however the system did not account for user behaviour and preference. A simple user model was used for relevance estimation, however these user models were static for the most part. Moreover, consumer fairness independent of the utility or general model performance was not a consideration. Merinov \cite{p42-merinov2023sustainability} began to explore sustainability-oriented tourism recommendation where the goals of the system included the mitigation of POI overcrowding, and the reduction of popularity bias. The stakeholder objective was modelled as an environment utility term, which serves as an aggregation of provider utilities, as well as a penalty for overcrowding. However, this aggregation risks accidentally encouraging the model to focus on a "small, diverse set" of POIs, which might globally reduce the popularity bias, but might still ignore some of the providers in the tail end of the distribution. With this lack of research in integrating both considerations at the same time, our goal for the research project thus involves integrating both consumer and provider fairness into a single methodology, as well as determining its efficacy in steering the model's metrics towards the objectives we lay out.


==> sections/results2.tex <==

\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[T]{0.42\textwidth}
         \centering
            % \includegraphics[width=\textwidth]{images/results_2/precision_vs_provider_alpha.png}
            % \caption{Precision@10 v.s. Provider fairness factor $\alpha$}
            \includegraphics[width=\textwidth]{images/results_2/exposure_long_tail_vs_provider_alpha.png}
            \caption{Long-tail Exposure v.s. Provider fairness factor $\alpha$}
            \label{fig:exp-longtail-provfactor}
     \end{subfigure}
     \begin{subfigure}[T]{0.44\textwidth}
         \centering
            \includegraphics[width=\textwidth]{images/results_3/precision_vs_consumer_beta.png}
            \caption{Precision@10 v.s. Consumer fairness factor $\beta$}
            \label{fig:prec-consfactor}
     \end{subfigure}


        \caption{Impact of the provider and consumer fairness factors separately}
\label{fig:provider-fairness}
\end{figure*}

\begin{figure*}[ht!]
\hspace*{\fill}%
     \centering
     \begin{subfigure}[T]{0.3\textwidth}
         \centering
            \includegraphics[width=\textwidth]{images/tradeoff_scatter_yelp.png}
     \end{subfigure}
     \hfill 
     \begin{subfigure}[T]{0.3\textwidth}
         \centering
            \includegraphics[width=\textwidth]{images/tradeoff_scatter_gowalla.png}
        \end{subfigure}
        \hspace*{\fill}%
    \caption{Scatterplot showing the tradeoff between GCE for users, GCE for items, and precision}
    \label{fig:tradeoff-scatter}
\end{figure*}

% \begin{figure*}[ht!]
%      \centering
%      \begin{subfigure}[T]{0.44\textwidth}
%          \centering
%     % \includegraphics[width=\textwidth]{images/results_3/mean_median_distance_vs_consumer_beta.png}
%     % \caption{Median POI distance v.s. Consumer fairness factor $\beta$}
%         % \label{fig:mmd-cons-fairness}
%                 \centering
%             \includegraphics[width=\textwidth]{images/results_3/precision_inactive_users_vs_consumer_beta.png}
%             \caption{Precision@10 for inactive users}
%             \label{fig:prec-consfactor-inactive}

%      \end{subfigure}


%         \caption{Impact of the consumer fairness factor}
% \label{fig:consumer-fairness}
% \end{figure*}
% \subsection{Comparison between exposure models}

The benchmark models were run first without modification, then while slowly increasing the provider fairness factor's coefficient $\alpha$ as outlined above. The impact of the provider fairness model used is first assessed by taking note of its impact on the precision and exposure metrics for the long tail, which it is aiming to improve. The results are shown below in Table \ref{table:prec-ltexp-exposuremodel-yelp}.


The score of the best-performing exposure model for the metric is highlighted in bold. For precision, which is the accuracy or performance metric of choice here, the linear exposure model performs the best in most cases. This makes sense as it doesn't punish even slightly popular POIs as harshly as the other models, as shown by the curves in Figure \ref{fig:different-models} in the appendix. Likewise, the logistic model performs the best in terms of exposure to the long tail, which makes sense as it only provides weights to only the least popular POIs. However, note that the linear model still provides a reasonable increase to the long-tail exposure as the weight increases. The power law model, however, seems to perform the worst for the GeoSoCa and LORE models and even decreases past a certain weight. Running a Kruskal-Wallis test on the precision and exposure values reveals a statistically significant difference in metric values among the 3 exposure models, starting from a factor weight of $\alpha = 0.5$, indicating that the choice of the exposure model does make a difference in the precision and long-tail exposure metrics. We can now use the linear model for the provider fairness factor, as it offers the highest precision values and permits moderate long-tail exposure.

\subsection{Impact of the provider fairness factor}
After adopting the linear model as the provider fairness factor for further analysis, its effects on performance metrics were thoroughly evaluated. As displayed in the previous table, increasing 
$a$ typically leads to a decline in precision. However, we see that it does help with exposure to the long-tail POIs, who under the normal regime experience very low exposure rates of 1-2 recommendation appearances overall. For USG, this exposure is as low as near-0 by default. As shown in Figure \ref{fig:exp-longtail-provfactor}, an increase in the factor's weight increases the long-tail exposure, reaching up to 1.4 times the default for GeoSoCa and LORE, and an even larger increase for the USG model.

% Figure \ref{fig:mmd-provider-fairness} captures the geographical implications of adjusting the fairness factor. Surprisingly, the median distance of recommended POIs relative to the user’s position remains relatively stable or even decreases with higher 
% $a$ values, particularly in the Gowalla dataset. This observation suggests that enhancing fairness by favouring less popular POIs does not necessarily compromise the geographical convenience of recommendations. These two figures collectively reveal the nuanced impact of integrating a provider fairness factor into the recommender system. While adjustments to $a$ influence precision across different models (GeoSoCa, LORE, USG) in varying degrees, they do not adversely affect the recommendations' geographical relevance. This comprehensive analysis underscores the importance of considering multiple metrics when evaluating the implications of fairness enhancements in recommender systems.
\subsection{Impact of the consumer fairness factor}
Increasing the weight of the consumer fairness factor, denoted as $\beta$, primarily aims to enhance precision for inactive users without affecting active users, as shown in Figures \ref{fig:prec-consfactor}. In the Yelp dataset, adjusting $\beta$ initially raises precision for the GeoSoCa and LORE models from 2.3\% to 2.6\%, but further increases lead to performance degradation, especially in the USG model, where precision drops from 3.0\% to 2.8\%. A Wilcoxon signed rank test confirms that even a slight increase in $\beta$ causes significant changes in precision across models, highlighting the sensitivity of recommender systems to fairness adjustments.

% \begin{figure}[!htb]
%     \centering
%     \makebox[\textwidth][c]{
%         \begin{minipage}{0.35\paperwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/results_3/precision_vs_consumer_beta.png}
%             \caption{Precision@10}
%             \label{fig:prec-consfactor}
%         \end{minipage}
%         \begin{minipage}{0.35\paperwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/results_3/ndcg_vs_consumer_beta.png}
%             \caption{NDCG@10}
%             \label{fig:ndcg-consfactor}
%         \end{minipage}
%     }
%     \makebox[\textwidth][c]{
%         \begin{minipage}{0.35\paperwidth}
%             \centering
%             \includegraphics[width=\textwidth]{images/results_3/precision_inactive_users_vs_consumer_beta.png}
%             \caption{Precision@10 for inactive users}
%             \label{fig:prec-consfactor-inactive}
%         \end{minipage}
%     }
%     \caption{Accuracy metrics v.s. Consumer fairness factor $\beta$}
%     \label{fig:acc-consfactor}
% \end{figure}


% If we use the same scatter visualization for consumer fairness in Figure \ref{fig:cons-fairness-scatter}, we see that the impact is a lot less directly positive, and the unfairness is much larger, as the points are further away from the blue line. For some models like USG, the factor even increases unfairness, as we also see in the plots above. Note that, because the strategy only affects inactive users, the factor does not affect the precision for active users, hence the points staying in the same line parallel to the x-axis.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.70\textwidth]{images/consumer_fairness_plot.png}
%     \caption{Plot of precision between the 2 consumer groups. The blue line represents perfect fairness where the values are the same.}
%     \label{fig:cons-fairness-scatter}
% \end{figure}


\subsection{Tradeoff between provider and consumer fairness}

Naturally, the effect of the combination of provider and consumer fairness factors on performance metrics can be assessed. A closer look at the GCE metrics for fairness for different tradeoffs is displayed in Figure \ref{fig:tradeoff-scatter}, which plots the tradeoff between the user precision GCE and the item exposure GCE metrics, while using color to denote precision, and shape to differentiate between models and values of $k$. These 2 plots are shown for both the Yelp and Gowalla datasets. In the left plot, we can see that the pareto front with respect to users GCE and items GCE, which goes around the upper right region of the plot, does not optimize for precision, and in fact consists of points that acheive low precision. Another thing to note is that the USG model seems to achieve the best precision, but at the cost of GCE for items. Luckily, this model as we've seen before is receptive to the provider fairness factor, even if its fairness often pales in comparison to other models. In the right plot, we see a similar story where the pareto front consists of models that achieve low precision. However, the points are a lot more spread out in this dataset, and some models like LORE are able to achieve moderate precision with a nice balance of the 2 fairness measures. This shows that the dataset and chosen model plays a significant role in how these 2 factors affect the recommendation quality. Certain models can have different baseline fairness measures and can respond differently to weight increase, while certain datasets can have users and properties that require a different provider or consumer fairness strategy, causing differences in how the weights affect where in the fairness plot the point goes.
